METCC: METric learning for Confounder Control Making distance matter in high dimensional biological analysis

High-dimensional data acquired from biological experiments such as next generation sequencing are subject to a number of confounding effects. These effects include both technical effects, such as variation across batches from instrument noise or sample processing, or institution-specific differences in sample acquisition and physical handling, as well as biological effects arising from true but irrelevant differences in the biology of each sample, such as age biases in diseases. Prior work has used linear methods to adjust for such batch effects. Here, we apply contrastive metric learning by a non-linear triplet network to optimize the ability to distinguish biologically distinct sample classes in the presence of irrelevant technical and biological variation. Using whole-genome cell-free DNA data from 817 patients, we demonstrate that our approach, METric learning for Confounder Control (METCC), is able to match or exceed the classification performance achieved using a best-in-class linear method (HCP) or no normalization. Critically, results from METCC appear less confounded by irrelevant technical variables like institution and batch than those from other methods even without access to high quality metadata information required by many existing techniques; offering hope for improved generalization.

==> figures/hcp_hyperparameters.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim={1cm 0 0 0}, clip]{figures/hcp_covariate_structure_regularization.png}
    \caption{regularization of covariate loading matrix $B$}
    \label{hcp_covariate_regularization}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim={1.1cm 0 0 0}, clip]{figures/hcp_global_structure_weight.png}
    \caption{regularization of global structure loading matrix $W$}
    \label{hcp_global_weight}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim={1cm 0 0 0}, clip]{figures/hcp_covariate_structure_weight.png}
    \caption{weight of known covariate loss term, $FB$ \imran{FB or just F?}}
    \label{hcp_covariate_weight}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth, trim={0.9cm 0 0 0}, clip]{figures/hcp_n_components.png}
    \caption{number of components in global structure matrix $X$}
    \label{hcp_n_components}
    \end{subfigure}
    \caption{HCP hyperparameters assessed over the grid, n components: [0, 50],
            $FB $loss weight: [0,200],
            $W$ regularization: [0, 75],
            $B$ regularization: [0, 30].
    The y-axis depicts hold-out AUC. \imran{put axis labels in the figures} Final parameters
    chosen are: regularization of $B=14$, regularization of $W=14$, 
    $FB$ loss weight $=12$, number of components in $X$ matrix $=3$}. \adam{Remove curve fits}
    \label{fig:hcp_perparameters}
\end{figure}

==> figures/metcc_hyperparameters.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth} 
    \includegraphics[width=\textwidth]{figures/metcc_dropout.png}
    \caption{p(dropout)}
    \label{metcc_dropout}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/metcc_neuron.png} 
    \caption{number of neurons in hidden layer}
     \label{metcc_neuron}
    \end{subfigure}
    \caption{\Methodname\ hyperparameter sweep. The y-axis depicts hold-out AUC. \imran{label your axes} Final
    parameters chosen are: batch size $=16$, number of neurons $=128$, learning rate =$1e-3$,
    p(dropout) $=0.4$, weight decay $=1e-5$}. \imran{this is a 2-d grid search, right? do 1-d plots even make sense here? (i'd think there might be interaction between the terms)}
    \label{fig:metcc_hyperparameters}
\end{figure}

==> tables/confounder_table.tex <==
\begin{table*}
  \centering
  \begin{tabular}{l|l|rrrr}
    \toprule
    \textbf{Normalization} & \textbf{Covariate} & \textbf{Train ACC} & \textbf{Train ACC std} &
    \textbf{Test ACC} & \textbf{Test ACC std} \\
   \midrule
     PCA-only (1)  & institution & \num{0.6617} & \num{0.0082} & \num{0.6617} & \num{0.0082} \\ 
    HCP (1) & institution & \num{0.8686} & \num{0.0060} & \num{0.8686} & \num{0.0060}\\
    \Methodname\ (1) & institution & \num{0.3875} & \num{0.0099} & \num{0.3875} & \num{0.0099}  \\

    Majority class  & institution &  
 \\ 
    \midrule
    PCA-only (1)  & flowcell & \num{0.2501} & \num{0.0092} & \num{0.2501} & \num{0.00929} \\ 
    HCP (1) & flowcell & \num{0.9090} & \num{0.0067} & \num{0.9090} & \num{0.0067}\\
    \Methodname\ (1) & flowcell & \num{0.07833} & \num{0.00417} & \num{0.07833} & \num{0.00417}  \\

    Majority class  & flowcell &  
 \\ 
    
    \midrule
    PCA-only  & age bin &  \num{0.2052} & \num{0.0057} & \num{0.169} & \num{0.0346}     \\ 
    HCP & age bin &  \num{1.0} & \num{0.0} & \num{0.1713} & \num{0.0418} \\ 
    \Methodname\  & age bin & \num{0.1616} & \num{0.0036} & \num{0.1617} & \num{0.032} \\ 
    Majority class  & age bin &  \num{0.1616} & \num{0.0036} & \num{0.1872} & \num{0.0282} \\ 
    \bottomrule
    \end{tabular}
      \caption{k-fold classification of confounder label for different normalization techniques}
  \label{table:cpt_stats}
\end{table*}


==> text/beyond.tex <==
 we apply technique that doesn't require full knowledge of known or unknown confounders
 
 the technique would only improve with larger sample counts
 
 can be used in a larger network with multiple loss functions or multitask learning, or other techniques that would generate augmenting data
 
 
 
